How to Color a French Flag--Biologically Inspired Algorithms for Scale-Invariant Patterning

In the French flag problem, initially uncolored cells on a grid must differentiate to become blue, white or red. The goal is for the cells to color the grid as a French flag, i.e., a three-colored triband, in a distributed manner. To solve a generalized version of the problem in a distributed computational setting, we consider two models: a biologically-inspired version that relies on morphogens (diffusing proteins acting as chemical signals) and a more abstract version based on reliable message passing between cellular agents. Much of developmental biology research has focused on concentration-based approaches using morphogens, since morphogen gradients are thought to be an underlying mechanism in tissue patterning. We show that both our model types easily achieve a French ribbon - a French flag in the 1D case. However, extending the ribbon to the 2D flag in the concentration model is somewhat difficult unless each agent has additional positional information. Assuming that cells are are identical, it is impossible to achieve a French flag or even a close approximation. In contrast, using a message-based approach in the 2D case only requires assuming that agents can be represented as constant size state machines. We hope that our insights may lay some groundwork for what kind of message passing abstractions or guarantees, if any, may be useful in analogy to cells communicating at long and short distances to solve patterning problems. In addition, we hope that our models and findings may be of interest in the design of nano-robots.

==> hybrid.tex <==
\section{Proposed Hybrid Model}
\label{sec:model_tradeoffs}

Previous work suggests a biologically interesting tradeoff between speed and robustness \cite{Navlakha2014}.
To probe this tradeoff, we propose a hybrid model in the French ribbon framework that is a combination of the concentration and message passing models, modified to consider noisy readings of gradient values $\lambda(C)$. In this model, a line graph of $n$ synchronous agents not only obtain $x$-coordinate information from a noisy gradient function, but can also engage in reliable, synchronous message passing with their neighbors.

Assume that in the hybrid model, the average morphogen concentration is described by the monotonically increasing
%\abnote{linear? identity?}
function $M(x)$, with threshold values $T_1$ and $T_2$ such that in the limit of zero noise, agents with $M(x) \leq T_1$ color blue, agents with $T_1 < M(x) \leq T_2$ color white, and agents with $M(x) > T_2$ color red.
The assumption of Gaussian distributions over position given noisy readings of the morphogen gradient has been empirically validated in previous work \cite{Dubuis2013}.
We assume that for an agent at $x$, the measured value $m = M(x)$ is normally distributed with mean $\mu$ and variance $\sigma^2$. Our goal is to show that by using message passing to correct errors around the threshold, we can achieve a correct ribbon with high probability.
\medskip

%{\em For additional convenience, we will assume that $\mu = x$, which we can obtain by setting the gradient function to simply be the identity.}

%\abnote{May be helpful to assume $\mu = x$ (so the gradient function is linear with slope 1 intercept 0) to do other stuff with the Gaussian for which $m$ is the noisy R.V.}

The following protocol suggests a tradeoff between robustness and time complexity in this hybrid model.
Say that agents sense their local concentrations $m = M(x)$ and, having some knowledge of
%the gradient function as well as
the thresholds, compute their color as blue if $m \leq T_1$, white if $T_1 < m \leq T_2$, and blue if $m > T_2$.
%Then, if for some fixed $\epsilon$, agents with $p(``blue"|m) > \epsilon$ color blue, agents with $p(``red"|m) > \epsilon$ color red, agents with both $p(``blue"|m) < 1-\epsilon$ and $p(``red"|m) < 1-\epsilon$ color white \abnote{these might be off, should consider single boundary case to start}, and the rest remain uncertain. At this point, the agents colored are correct with probability $1-\epsilon$.
%\abnote{define an indicator var to count uncertain agents? and show that this sum depends on $\sigma$?}
In the next phase, agents communicate their states to their neighbors. Consider one of the two thresholds in the three-color case. At this threshold, say the minimum-size interval containing all uncertain agents has size $s$. Assuming reliable and synchronous message passing, this interval can be learned by all the agents it contains in $O(s)$, and all agents within the interval can be marked as uncertain. Then, agents color the uncertain interval in $O(s)$, simply by having uncertain agents yield to the first color they receive from an agent outside the interval. \abnote{hm, do we need to prove this works}
%\abnote{this protocol just means that the uncertain interval is decided by the two endpoints of the uncertain interval, and any decided agents in the interval should become uncertain again?}
% \fnote{Given knowledge of the noise distribution and the gradient function, each agent can . }



To analyze the proportion of agents who color correctly, we compute the posterior probabilities:
\begin{itemize}
    \item $\Pr{``blue"|m} = \Pr{x < M^{-1}(T_1) | m}$
    \item $\Pr{``white"|m} = \Pr{M^{-1}(T_1) < x < M^{-1}(T_2) | m}$
    \item $\Pr{``red"|m} = \Pr{x > M^{-1}(T_2) | m}$
\end{itemize}

Since $s$ depends on $\sigma^2$, there is a tradeoff between robustness (i.e. potential for error correction) and time in this noisy French ribbon formulation. While we are not guaranteed that $s << n$, leaving $O(n)$ and $O(s)$ asymptotically comparable, \abnote{todo - finish}


==> preamble.tex <==
%% Courtesy: Daniel Spielman, via Madhu Sudan --> Vinod Vaikuntanathan --> Aloni Cohen

%--------------
%% preamble.tex
%% this should be included with a command like
%% \input{preamble.tex}
%% \lecture{1}{September 4, 1996}{Daniel A. Spielman}{name
%%  of poor scribe}

\hbadness=10000
\vbadness=10000

\newcommand{\handout}[6]{
   \renewcommand{\thepage}{\Large\bf #2 / Page \arabic{page}}
   \noindent
   \begin{center}
   \framebox{
      \vbox{
    \hbox to 5.78in { {\bf #1}
     	 \hfill #3 }
       \vspace{4mm}
       \hbox to 5.78in { {\Large \hfill #6  \hfill} }
       \vspace{2mm}
       \hbox to 5.78in { {\it #4 \hfill #5} }
      }
   }
   \end{center}
   \vspace*{4mm}
}

% \newtheorem{theorem}{Theorem}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{observation}[theorem]{Observation}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{claim}[theorem]{Claim}
% \newtheorem{fact}[theorem]{Fact}
% \newtheorem{assumption}[theorem]{Assumption}
% \newtheorem{assertion}[theorem]{Assertion}
% \def\figureautorefname{Figure}
% \def\tableautorefname{Table}%
% \def\partautorefname{Part}%
% \def\chapterautorefname{Chapter}%
% \def\sectionautorefname{Section}%
% \def\subsectionautorefname{Section}%
% \def\subsubsectionautorefname{Section}%
% \def\algorithmautorefname{Algorithm}%


\def\NewTheorem#1#2{%
  \newaliascnt{#1}{theorem}
  \newtheorem{#1}[#1]{#2}
  \aliascntresetthe{#1}
  \expandafter\def\csname #1autorefname\endcsname{#2}
}


 \newtheorem{theorem}{Theorem}[section]
\NewTheorem{lemma}{Lemma}
\NewTheorem{corollary}{Corollary}
\NewTheorem{definition}{Definition}
\NewTheorem{remark}{Remark}



\NewTheorem{conjecture}{Conjecture}
\NewTheorem{observation}{Observation}
\NewTheorem{assumption}{Assumption} 
\NewTheorem{assumptions}{Assumptions} 


\NewTheorem{proposition}{Proposition}

\NewTheorem{claim}{Claim}
\newtheorem{notation}{Notation}
\newtheorem*{idea}{Proof (sketch)}
\theoremstyle{remark}
\newtheorem{boldclaim}{Bold claim}
\renewcommand*{\figureautorefname}{Figure}%
\renewcommand*{\tableautorefname}{Table}%
%\renewcommand*{\partautorefname}{Part}%
%\renewcommand*{\chapterautorefname}{Chapter}%
\renewcommand*{\sectionautorefname}{Section}%
\renewcommand*{\subsectionautorefname}{Section}%
\renewcommand*{\subsubsectionautorefname}{Section}%



%%%% GENERAL COMMANDS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\ripref}[2]{ \it \hyperref[#2]{\it #1}~\ref{#2}    }
\newcommand{\dist}{\operatorname{dist}}
\newcommand{\dis}{\mathop{\mbox{\rm d}}\nolimits}
\newcommand{\per}{\mathop{\mbox{\rm per}}\nolimits}
\newcommand{\area}{\mathop{\mbox{\rm area}}\nolimits}
\newcommand{\cw}{\mathop{\rm cw}\nolimits}
\newcommand{\ccw}{\mathop{\rm ccw}\nolimits}
\newcommand{\DIST}{\mathop{\mbox{\rm DIST}}\nolimits}
\newcommand{\OP}{\mathop{\mbox{\it OP}}\nolimits}
\newcommand{\OPprime}{\mathop{\mbox{\it OP}^{\,\prime}}\nolimits}
\newcommand{\ihat}{\hat{\imath}}
\newcommand{\jhat}{\hat{\jmath}}
%\newcommand{\abs}[1]{\mathify{\left| #1 \right|}}


%%%%% PROOF ENVIRONMENTS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newenvironment{proof-sketch}{\noindent{\bf Sketch of Proof}\hspace*{1em}}{\qed\bigskip}
\newenvironment{proof-idea}{\noindent{\bf Proof Idea}\hspace*{1em}}{\qed\bigskip}
\newenvironment{proof-of-lemma}[1]{\noindent{\bf Proof of Lemma #1}\hspace*{1em}}{\qed\bigskip}
\newenvironment{proof-attempt}{\noindent{\bf Proof Attempt}\hspace*{1em}}{\qed\bigskip}
\newenvironment{proofof}[1]{\noindent{\bf Proof}
of #1:\hspace*{1em}}{\qed\bigskip}
% \newenvironment{remark}{\noindent{\bf Remark}\hspace*{1em}}{\bigskip}

% \makeatletter
% \@addtoreset{figure}{section}
% \@addtoreset{table}{section}
% \@addtoreset{equation}{section}
% \makeatother

\newcommand{\FOR}{{\bf for}}
\newcommand{\TO}{{\bf to}}
\newcommand{\DO}{{\bf do}}
\newcommand{\WHILE}{{\bf while}}
\newcommand{\AND}{{\bf and}}
\newcommand{\IF}{{\bf if}}
\newcommand{\THEN}{{\bf then}}
\newcommand{\ELSE}{{\bf else}}

% \renewcommand{\thefigure}{\thesection.\arabic{figure}}
% \renewcommand{\thetable}{\thesection.\arabic{table}}
% \renewcommand{\theequation}{\thesection.\arabic{equation}}

\makeatletter
\def\fnum@figure{{\bf Figure \thefigure}}
\def\fnum@table{{\bf Table \thetable}}
\long\def\@mycaption#1[#2]#3{\addcontentsline{\csname
  ext@#1\endcsname}{#1}{\protect\numberline{\csname
  the#1\endcsname}{\ignorespaces #2}}\par
  \begingroup
    \@parboxrestore
    \small
    \@makecaption{\csname fnum@#1\endcsname}{\ignorespaces #3}\par
  \endgroup}
\def\mycaption{\refstepcounter\@captype \@dblarg{\@mycaption\@captype}}
\makeatother


\newcommand{\figcaption}[1]{\mycaption[]{#1}}
\newcommand{\tabcaption}[1]{\mycaption[]{#1}}
\newcommand{\head}[1]{\chapter[Lecture \##1]{}}
\newcommand{\mathify}[1]{\ifmmode{#1}\else\mbox{$#1$}\fi}
%\renewcommand{\Pr}[1]{\mathify{\mbox{Pr}\left[#1\right]}}
%\newcommand{\Exp}[1]{\mathify{\mbox{Exp}\left[#1\right]}}
\newcommand{\bigO}O
\newcommand{\set}[1]{\mathify{\left\{ #1 \right\}}}
\def\half{\frac{1}{2}}


% Command that ignores input.
\newcommand{\remove}[1]{}
\newcommand{\ignore}[1]{}
\newenvironment{ignoreme}{\ignore{}{}}

%%%%%%%%%%%%%% LATTICES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\def\hh{\sigma^{\text{\rm\tiny top}}}
\def\ph{\sigma^{\text{\rm\tiny bot}}}
\def\hM{M^{\text{\rm\tiny top}}}
\def\pM{M^{\text{\rm\tiny bot}}}
\def\lsb{\mathsf{lsb}}

\newcommand{\gapSVP}{\mathsf{gapSVP}}
\newcommand{\SIVP}{\mathsf{SIVP}}

\def\dlwe{\mathsf{DLWE}}


\def\Zp{\Z_p}
\newcommand{\ip}[1]{\langle #1 \rangle}
\def\Psibar{\overline{\Psi}}

%Security Parameter
\newcommand{\secparam}{\kappa}
\newcommand{\secp}{\secparam}

\newcommand{\svp}{\mathsf{SVP}}

% Vectors, Matrices and such

\def\veca{\vc{a}}
\def\vecb{\vc{b}}
\def\vecc{\vc{c}}
\def\vecd{\vc{d}}
\def\vece{\vc{e}}
\def\vecm{\vc{m}}
\def\vecs{\vc{s}}
\def\vect{\vc{t}}
\def\vecv{\vc{v}}
\def\vecx{\vc{x}}
\def\vecy{\vc{y}}

\def\Z{\mathbb{Z}}
\def\N{\mathbb{N}}
\def\R{\mathbb{R}}
\def\Q{\mathbb{Q}}

% Changing QED symbol in claim proofs
\newenvironment{claimproof}{\begin{proof}
\renewcommand{\qedsymbol}{{$\blacksquare$}}
}{\end{proof}}

% Calligraphic and blackboard type letters.

\def\cA{{\cal A}}
\def\cB{{\cal B}}
\def\cC{{\cal C}}
\def\cD{{\cal D}}
\def\cE{{\cal E}}
\def\cF{{\cal F}}
\def\cG{{\cal G}}
\def\cH{{\cal H}}
\def\cI{{\cal I}}
\def\cJ{{\cal J}}
\def\cK{{\cal K}}
\def\cL{{\cal L}}
\def\cM{{\cal M}}
\def\cN{{\cal N}}
\def\cO{{\cal O}}
\def\cP{{\cal P}}
\def\cQ{{\cal Q}}
\def\cR{{\cal R}}
\def\cS{{\cal S}}
\def\cT{{\cal T}}
\def\cU{{\cal U}}
\def\cV{{\cal V}}
\def\cW{{\cal W}}
\def\cX{{\cal X}}
\def\cY{{\cal Y}}
\def\cZ{{\cal Z}}
%%%%%%%%%%%%%%%%%
\def\bbC{{\mathbb C}}
\def\bbE{{\mathbb E}}
\def\bbF{{\mathbb F}}
\def\bbG{{\mathbb G}}
\def\bbM{{\mathbb M}}
\def\bbN{{\mathbb N}}
\def\bbQ{{\mathbb Q}}
\def\bbR{{\mathbb R}}
\def\bbV{{\mathbb V}}
\def\bbZ{{\mathbb Z}}

\def\Zq{\bbZ_q}

%%%%%%%%%%%%%%%%%


% Rounding commands

\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\round}[1]{\left\lfloor #1 \right\rceil}


% Other short-hands

\def\binset{\{0,1\}}
\def\pmset{\{\pm 1\}}
\def\ind{\mathbbm{1}}
%\def\ind{\mathbf{1}}

%\newcommand{\norm}[1]{\left\| {#1} \right\|}
\newcommand{\norminf}[1]{\left\| {#1} \right\|_{\infty}}


% Assignments
\def\getsr{\stackrel{\scriptscriptstyle{\$}}{\gets}}
\def\getsd{{:=}}
%\def\bydef{\stackrel{.}{=}}
\def\bydef{\triangleq}
\def\getsf{{\gets}}



% Asymptotics

\def\poly{{\rm poly}}
\def\polylog{{\rm polylog}}
\def\polyloglog{{\rm polyloglog}}
\def\negl{{\rm negl}}
\newcommand{\ppt}{\mbox{{\sc ppt}}}
\def\Otilde{\widetilde{O}}

% Indistinguishability
\newcommand{\cind}{{\ \stackrel{c}{\approx}\ }}
\newcommand{\sind}{{\ \stackrel{s}{\approx}\ }}

% Complexity classes

\def\NP{\mathbf{NP}}
\def\Ppoly{{\mathbf{P}/\poly}}


% Cryptographic assumptions

\newcommand{\ddh}{\mathrm{DDH}}
\newcommand{\cdh}{\mathrm{CDH}}
\newcommand{\dlin}{\text{\rm $d$LIN}}
\newcommand{\lin}{\text{\rm Lin}}
\newcommand{\sxdh}{\mathrm{SXDH}}
\newcommand{\rsa}{\mathrm{RSA}}
\newcommand{\sis}{\mathrm{SIS}}
\newcommand{\isis}{\mathrm{ISIS}}
\newcommand{\lwe}{\mathsf{LWE}}
\newcommand{\qr}{\mathrm{QR}}


% Types of attacks

\newcommand{\adv}{\mathrm{Adv}}
\newcommand{\dst}{\mathrm{Dist}}
\newcommand{\leak}{\mathrm{Leak}}
\newcommand{\forge}{\mathrm{Forge}}
\newcommand{\col}{\mathrm{Col}}
\newcommand{\invt}{\mathrm{Inv}}
\newcommand{\cpa}{\text{\rm CPA}}
\newcommand{\kdm}{\mathrm{KDM}}
\newcommand{\kdi}{\mathrm{KDM}^{(1)}}
\newcommand{\kdmn}{\mathrm{KDM}^{(\usr)}}
\newcommand{\ibe}{\mathrm{IBE}}
\newcommand{\good}{\mathrm{GOOD}}
\newcommand{\legal}{\mathrm{L}}


% Quadratic residuosity related

\newcommand{\qrs}{\mathbb{QR}}
\newcommand{\js}{\mathbb{J}}


% Linear algebra

\newcommand{\mx}[1]{\mathbf{{#1}}}
\newcommand{\vc}[1]{\mathbf{{#1}}}
\newcommand{\gvc}[1]{\bm{{#1}}}
%\newcommand{\vc}[1]{\gvc{{#1}}}

\newcommand{\rk}{\text{\rm Rk}}
\newcommand{\spn}{\text{\rm Span}}

% Probability

\newcommand{\Ex}{\mathop{\bbE}}
\newcommand{\cov}{\mathop{\text{\rm Cov}}}

%\newcommand{\sd}{\mathop{\text{\tt dist}}}
\newcommand{\sd}{\mathop{\Delta}}


% Entropy

\newcommand{\mH}{\mathbf{H_{\infty}}}
\newcommand{\avgmH}{\mathbf{\widetilde{H}_{\infty}}}


% Cryptographic elements

\newcommand{\pk}{{pk}}
\newcommand{\evk}{{evk}}
%\newcommand{\pp}{{pp}}
\newcommand{\sk}{{sk}}
\newcommand{\vk}{{vk}}
\newcommand{\td}{{td}}

\newcommand{\msk}{{msk}}
%\newcommand{\id}{{id}}

\newcommand{\crs}{\text{\sf crs}}

\newcommand{\params}{{params}}
\newcommand{\state}{{setupstate}}

\newcommand{\query}{{query}}
\newcommand{\qstate}{{qstate}}
\newcommand{\resp}{{resp}}


% Algorithms


\newcommand{\keygen}{\mathsf{Keygen}}
\newcommand{\gen}{\mathsf{Gen}}
\newcommand{\eval}{\mathsf{Eval}}
\newcommand{\setup}{\mathsf{Setup}}
\newcommand{\extract}{\mathsf{Extract}}
\newcommand{\enc}{\mathsf{Enc}}
\newcommand{\dec}{\mathsf{Dec}}

\newcommand{\symname}{\mathsf{SYM}}
\newcommand{\symkeygen}{\mathsf{SYM.Keygen}}
\newcommand{\symgen}{\symkeygen}
\newcommand{\symenc}{\mathsf{SYM.Enc}}
\newcommand{\symdec}{\mathsf{SYM.Dec}}


\newcommand{\shname}{\mathsf{SH}}
\newcommand{\shkeygen}{\mathsf{SH.Keygen}}
\newcommand{\shgen}{\shkeygen}
\newcommand{\shenc}{\mathsf{SH.Enc}}
\newcommand{\shdec}{\mathsf{SH.Dec}}
\newcommand{\sheval}{\mathsf{SH.Eval}}

\newcommand{\hename}{\mathsf{HE}}
\newcommand{\hekeygen}{\mathsf{HE.Keygen}}
\newcommand{\hegen}{\hekeygen}
\newcommand{\heenc}{\mathsf{HE.Enc}}
\newcommand{\hedec}{\mathsf{HE.Dec}}
\newcommand{\heeval}{\mathsf{HE.Eval}}


\newcommand{\fhname}{\mathsf{FH}}
\newcommand{\fhkeygen}{\mathsf{FH.Keygen}}
\newcommand{\fhenc}{\mathsf{FH.Enc}}
\newcommand{\fhdec}{\mathsf{FH.Dec}}
\newcommand{\fheval}{\mathsf{FH.Eval}}

\newcommand{\btsname}{\mathsf{BTS}}
\newcommand{\btkeygen}{\mathsf{BTS.Keygen}}
\newcommand{\btgen}{\btkeygen}
\newcommand{\btenc}{\mathsf{BTS.Enc}}
\newcommand{\btdec}{\mathsf{BTS.Dec}}
\newcommand{\bteval}{\mathsf{BTS.Eval}}

\newcommand{\fhename}{\mathsf{FHE}}
\newcommand{\fhekeygen}{\mathsf{FHE.Keygen}}
\newcommand{\fhegen}{\fhekeygen}
\newcommand{\fheenc}{\mathsf{FHE.Enc}}
\newcommand{\fhedec}{\mathsf{FHE.Dec}}
\newcommand{\fheeval}{\mathsf{FHE.Eval}}



\newcommand{\kdmkeygen}{\mathsf{KDM.Keygen}}
\newcommand{\kdmenc}{\mathsf{KDM.Enc}}
\newcommand{\kdmdec}{\mathsf{KDM.Dec}}

\newcommand{\vssgen}{\mathsf{VSS.Gen}}

\newcommand{\pirname}{\mathsf{PIR}}
\newcommand{\pirsetup}{\mathsf{PIR.Setup}}
\newcommand{\pirquery}{\mathsf{PIR.Query}}
\newcommand{\piranswer}{\mathsf{PIR.Response}}
\newcommand{\pirresp}{\piranswer}
\newcommand{\pirdec}{\mathsf{PIR.Decode}}
\newcommand\E[1]{\mathbb{E}\left[\,#1\,\right]}
\renewcommand{\Pr}[1]{\mathbb{P}\left[\,#1\,\right]}




% Document specific definitions

\newcommand{\idl}[1]{\left\langle{#1}\right\rangle}
\newcommand{\rlwe}{\mathsf{RLWE}}
\newcommand{\plwe}{\mathsf{PLWE}}
\newcommand{\drlwe}{\text{\rm G-RLWE}}
\newcommand{\sdrlwe}{\text{\rm RLWE}}
\newcommand{\vssm}{\text{\rm SVSS}}

\newcommand{\ekdm}{{\cE_{\kdm}}}
\newcommand{\usr}{{\nu}}

\newcommand{\add}{\mathsf{add}}
\newcommand{\mlt}{\mathsf{mult}}

\newcommand{\hc}{\hat{c}}

\newcommand{\otild}{{\widetilde{O}}}
\newcommand{\omtild}{{\widetilde{\Omega}}}

\newcommand{\linf}{{\ell_{\infty}}}

\newcommand{\gf}{{\text{GF}}}

\newcommand{\zset}[1]{\{0, \ldots, {#1}\}}


\newcommand{\fig}[4]{
        \begin{figure}
        \setlength{\epsfysize}{#2}
        \vspace{3mm}
        \centerline{\epsfbox{#4}}
        \caption{#3} \label{#1}
        \end{figure}
        }

\newcommand{\ord}{{\rm ord}}

\providecommand{\norm}[1]{\lVert #1 \rVert}
\newcommand{\embed}{{\rm Embed}}
\newcommand{\qembed}{\mbox{$q$-Embed}}
\newcommand{\lp}{{\rm LP}}

\renewcommand{\eps}{\varepsilon}
